Linear genetic programming control for strongly nonlinear dynamics with frequency crosstalk

We advance Machine Learning Control (MLC), a recently proposed model-free control framework which explores and exploits strongly nonlinear dynamics in an unsupervised manner. The assumed plant has multiple actuators and sensors and its performance is measured by a cost functional. The control problem is to find a control logic which optimizes the given cost function. The corresponding regression problem for the control law is solved by employing linear genetic programming as an easy and simple regression solver in a high-dimensional control search space. This search space comprises open-loop actuation, sensor-based feedback and combinations thereof, thus generalizing former MLC studies. This methodology is denoted as linear genetic programming control (LGPC). Focus of this study is the frequency crosstalk between unforced unstable oscillation and the actuation at different frequencies. LGPC is first applied to the stabilization of a forced nonlinearly coupled three-oscillator model comprising open- and closed-loop frequency crosstalk mechanisms. LGPC performance is then demonstrated in a turbulence control experiment, achieving 22% drag reduction for a simplified car model. For both cases, LGPC identifies the best nonlinear control achieving the optimal performance by exploiting frequency crosstalk. Our control strategy is suited to complex control problems with multiple actuators and sensors featuring nonlinear actuation dynamics.

==> App1.tex <==
%SSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSSS
% =============== APPENDIX =======================================%
\section{Classical multidimensional scaling (CMDS)}
\label{Sec:App1:CMDS}
Classical multidimensional scaling (CMDS) is employed to visualize the similarity of control laws (see \S~\ref{ToC:LGPC}).
CMDS aims to find a low-dimensional representation of points $\boldsymbol\gamma^l$, $l=1,\ldots,N$, 
such that the average error between the distances between points $\boldsymbol\gamma^l$ and the elements of a given distance matrix $\boldsymbol{\mathsfbi{D}}$, 
here emulating the distance between the time series of different control laws, is minimal.

In order to find a unique solution to CMDS, 
we assume that $\boldsymbol{\Gamma}=[\boldsymbol{\gamma}^1\quad \boldsymbol{\gamma}^2\quad \ldots\quad\boldsymbol{\gamma}^N]$ with $\boldsymbol{\gamma}^1,\ldots,\boldsymbol{\gamma}^N\in\mathbb{R}^r$ is centered, 
i.e.\ $\boldsymbol{\Gamma}$ is a mean-corrected matrix with $1/N\,\sum_{l=1}^N\, \boldsymbol{\gamma}^l = [0 \ldots 0]^T$.
Rather than directly finding $\boldsymbol{\Gamma}$, we search for the Gram matrix 
$\boldsymbol{\mathsfbi{B}}=\boldsymbol{\Gamma}^T\boldsymbol{\Gamma}$ that is real, symmetric and positive semi-definite.
Since $\boldsymbol{\Gamma}$ is assumed to be centered, the Gram matrix is the Euclidean inner product, and we have 
$\mathsfi{D}_{lm}^2=\vert\vert \boldsymbol{\gamma}^l-\boldsymbol{\gamma}^m\vert\vert_2^2=\mathsfi{B}_{ll} + \mathsfi{B}_{mm} - 2\,\mathsfi{B}_{lm}$.
In the first step of the classical scaling algorithm, the matrix $\boldsymbol{\mathsfbi{D}}_2$ of elements $\left(\mathsfi{D}_2\right)_{lm} = -\frac{1}{2}\mathsfi{D}_{lm}^2$ is constructed.
Then, we form the "doubly centered" matrix  $\boldsymbol{\mathsfbi{B}} = \boldsymbol{\mathsfbi{C}}\boldsymbol{\mathsfbi{D}}_2\boldsymbol{\mathsfbi{C}}$, where $\boldsymbol{\mathsfbi{C}}=\boldsymbol{\mathsfbi{I}}_N-N^{-1}\boldsymbol{\mathsfbi{J}}_N$ with $\boldsymbol{\mathsfbi{I}}_N$ the identity matrix of size $N$ and $\boldsymbol{\mathsfbi{J}}_N$ an $N\times N$ matrix of ones. The term "doubly centered" refers to the subtraction of the row as well as the column mean.
Let the eigendecomposition of $\boldsymbol{\mathsfbi{B}}$ be $\boldsymbol{\mathsfbi{B}} = \boldsymbol{\mathsfbi{V}}\boldsymbol{\mathsfbi{\Lambda}}\boldsymbol{\mathsfbi{V}}^T$ 
where $\boldsymbol{\mathsfbi{\Lambda}}$ is a diagonal matrix with ordered eigenvalues
$\lambda_1\geq \lambda_2 \geq\ldots\geq\lambda_N\geq 0$
and $\boldsymbol{V}$ contains the eigenvectors as columns.
Then $\boldsymbol{\Gamma}$ can be recovered from
\begin{equation}
\boldsymbol{\Gamma} = \boldsymbol{\mathsfbi{\Lambda}}^{\frac{1}{2}}\boldsymbol{\mathsfbi{V}}^T.
\end{equation}
Having only the distance matrix, the resulting representation is only defined up 
to a translation, a rotation, and reflections of the axes.
If the distance matrix is computed using the Euclidean distance and all eigenvalues are non-negative,
$\boldsymbol{\Gamma}$ can be recovered.
If $r<N$, there exist $N-r$ zero eigenvalues, 
in which case a low-dimensional subspace can be found in which the presentation of $\boldsymbol{\Gamma}$ would be exact.
For other distance metrics, the distances of the presentation found by CMDS is an approximation to the true distances.
In this case, some eigenvalues may be negative and only the positive eigenvalues and their associated eigenvectors 
are considered to determine an approximative representation of $\boldsymbol{\Gamma}$.
Note that for the Euclidean distance metric, CMDS is closely related to a principal component analysis (PCA)
commonly used to find a low-dimensional subspace. 
While CMDS, and multi-dimensional scaling generally, uses a distance matrix as input, PCA is based on a data matrix.
A distance matrix $\boldsymbol{\mathsfbi{D}}$ can be directly computed for the centered matrix $\boldsymbol{\Gamma}$. 
If the Euclidean distance is employed for computing the distances, 
the result from applying CMDS to $\boldsymbol{\mathsfbi{D}}$ corresponds to the result 
from applying PCA to $\boldsymbol{\Gamma}$.
A proof can be found in \cite{Mardia1979book}.
The quality of the representation is typically measured by 
$\sum_{l=1}^r\,\lambda_l/\sum_{l=1}^{N-1}\,\lambda_l$, 
and more generally if $\boldsymbol{\mathsfbi{B}}$ is not positive semi-definite using
$\sum_{l=1}^r\,\lambda_l/\sum_{\lambda>0}\,\lambda_l$.

==> App2.tex <==
\section{A comparison between LGPC and TGPC}
\label{sec:comp_LGP_TGP}
In this section, a comparison between the LGPC and the traditional TGP control (referred to as TGPC hereafter) is performed.
Instead of evolving a matrix in LGP, the classical TGP evolves a binary tree-structure. 
The inner nodes of such trees hold operators ($+,-,\times,\div,$ \ldots).
The leaves hold sensors or constants.
Crossover is performed by exchanging two randomly chosen sub-trees of two individuals, while mutation replaces a sub-tree by a new random sub-tree.
Readers are referred to the literature \cite{Duriez2016book} for further details on TGPC.

For a fair comparison, TGPC is applied to the same control problem (Eq. \ref{eq:3osc}) with the similar parameter settings in Table \ref{tab:LGP_param}.
The tree-depth of individuals of initial population varies between 2 and 8 using a Gaussian distribution. 
Half the individuals have a full tree structure, \emph{i.e.} each leaf being forced to have the same prescribed depth. 
The maximum tree-depth for the whole population is forced to be 16.
Five independent runs were performed to provide a reasonably statistical comparison.
The comparison examines the following features:
\begin{itemize}
	\item \textbf{control performance}. The optimal cost value serves to quantify the performance. We denote by $(J_1^{N})_{\# k}$ the optimal cost value in the $k$th run.
	\item \textbf{complexity of programs}. A good indicator of the complexity is the number of executed operations as it is directly related to the computational load of each individual. This means a comparison between the number of inner nodes (which hold the operators) for TGPC and the number of effective instructions for LGPC.
	\item \textbf{rate of convergence}. This may be assessed from the evolution of the best cost value $J_1^n, n=1,\ldots,N$ and the median value $J_{\text{median}}^n, n=1,\ldots,N$ with increasing generations. The median value is chosen over the mean value as the latter could be strongly influenced by the worst individuals \cite{Duriez2016book}. An insight over the diversity of the population can be gained from the difference between best and median value.
\end{itemize}

We display the averaged results over 5 runs in table \ref{tab:comp_TGPC_LGPC} and Fig. \ref{fig:comp_conv}. 
Global complexity gives the averaged value obtained from the whole population of all runs ($5\times M \times N$), while the 1st complexity is only averaged over the best individual of 5 runs.
The averaged performance is similar for the two methods.
LGPC shows an advantage over TGPC in terms of the complexity.
...

Fig. \ref{fig:comp_conv} visualizes the rate of convergence of THE two methods. 
Despite of similar features in heading and ending generations, TGPC evolves quicker to better individuals than LGPC.







\begin{table}
	\centering	
\begin{tabular}{l | *{2}{c}}
	 & LGPC & TGPC\\ \hline
	 Control performance & $1.67\times10^{-3}$ & $1.62\times10^{-3}$\\
	Global complexity & 6 & 16\\
	1st complexity & 10 & 22\\
\end{tabular}
	\caption{Comparison between LGPC and TGPC. The results are averaged over 5 runs.}
	\label{tab:comp_TGPC_LGPC}
\end{table}


%--- Figure ------------------------------------------------------------
\graphicspath{{./Figures/}}
\begin{figure}
	\centering
	\includegraphics[scale = 0.5]{Comp_convergence.pdf}
	\caption{Comparison of the rate of convergence. The results are averaged over 5 runs.}
	\label{fig:comp_conv}
\end{figure} 
%---------------------------------------------------------------


